Enhancing SCADA Security: Developing a Host-Based Intrusion Detection System to Safeguard Against Cyberattacks

With the increasing reliance of smart grids on correctly functioning SCADA systems and their vulnerability to cyberattacks, there is a pressing need for effective security measures. SCADA systems are prone to cyberattacks, posing risks to critical infrastructure. As there is a lack of host-based intrusion detection systems specifically designed for the stable nature of SCADA systems, the objective of this work is to propose a host-based intrusion detection system tailored for SCADA systems in smart grids. The proposed system utilizes USB device identification, flagging, and process memory scanning to monitor and detect anomalies in SCADA systems, providing enhanced security measures. Evaluation in three different scenarios demonstrates the tool's effectiveness in detecting and disabling malware. The proposed approach effectively identifies potential threats and enhances the security of SCADA systems in smart grids, providing a promising solution to protect against cyberattacks.

==> chapter1.tex <==
\section{Introduction} \label{sec:introduction}
The advent of the \ac{iot} has led to its incorporation with \acp{cps}, enriching the operational capabilities of conventional \acp{sg}~\cite{jahromi2021toward}.
Furthermore, \ac{scada} systems have experienced substantial advancements across four generations, culminating in IoTization~\cite{yadav2021architecture}.
Such integrations within \ac{scada}, \ac{iot}, and cloud environments pave the way for cost-effectiveness, flexibility, and enhanced performance~\cite{babayigit2023industrial,henze2017distributed}.
However, this digital evolution blurs the boundaries between \ac{ot} and \ac{it} as well as between process and external networks, including the public Internet~\cite{rahman2022deep}.
This, in turn, significantly heightens the threat surface for potential intrusion by unauthorized third parties, necessitating a comprehensive security concept for \ac{scada} systems~\cite{krause2021cybersecurity}.

\ac{scada} systems, crucial for grid operation, are prone to cyberattacks, emphasizing the need for robust protective measures~\cite{khan2022enhancing}.
While typically insulated within demilitarized zones, these systems remain vulnerable to indirect malware propagation~\cite{van2020methods}, such as Stuxnet's USB drive insertion~\cite{iaiani2021analysis}.
The majority of research concentrates on Network-based \acp{ids}, neglecting \ac{scada}-specific \acp{hids}~\cite{rakas2020review,wolsing2022ipal}.
As \ac{scada}-focused malware often involves sophisticated, zero-day threats, this lack of attention on \ac{hids} is concerning~\cite{alanazi2022scada}.
\ac{hids} can excel in detecting new processes and external hardware insertions, offering a more comprehensive security setup alongside \ac{nids}~\cite{stoddart2022gaining}. 
However, specific research on \ac{hids} in \ac{scada} systems, especially concerning new, unknown processes and hardware insertions, remains limited. %, warranting this paper's focus.

Consequently, the development of a robust \ac{hids} for \ac{scada} applications is indispensable to safeguard against cyber threats.
More specifically, features such as detection of hardware insertion, e.g., USB device identification and flagging, alongside process memory scanning and hashing are required.
The complexity of the system and the increased interaction between different actors not only challenge cyber-physical sovereignty but also expose the system to a myriad of cyber threats~\cite{bader2023comprehensively}.
%
Addressing the mounting threats to \ac{scada} systems requires a two-pronged approach:
%
\begin{enumerate}[(i)]
\item The formulation of an effective methodology for detecting and identifying unknown processes within \ac{scada} system host environment.
\item The design of a robust and reliable \ac{hids} approach for providing high detection quality.
\end{enumerate}
%
Thus, the objective of this paper is to propose a comprehensive \ac{hids} for \ac{scada} systems, incorporating USB device identification, process memory scanning, and hashing, and demonstrate its efficiency through different scenarios, while evaluating its reliability.
%
The key contributions are:
%
\begin{enumerate}
\item A comprehensive overview of the present state of \ac{hids} for \ac{scada} systems, identifying gaps in current research.
\item A novel \ac{hids} for \ac{scada} systems, providing a reliable approach for protecting detecting unknown threats via malware.
\item Validation of \ac{hids} approach using different scenarios, demonstrating the effectiveness and reliability.
\end{enumerate}

==> chapter2.tex <==
\section{Cyber Security in Smart Grids} \label{sec:background}
To lay the foundation for our work, we first provide an overview of \ac{scada} system, then related work and problem analysis on \ac{hids}.
%
\subsection{\ac{scada} System} \label{sec:scada}
\ac{scada} systems, critical to grid operation, are prone to cyber threats such as Stuxnet, Duqu, and Conficker~\cite{alagappan2022augmenting}.
This susceptibility extends from human operators to localized communication devices within the control centers, indicating that a successful strike could disrupt the entire system.
The \ac{scada} system's unique structure encompasses a \ac{hmi}, supervisory system, \acp{rtu}, \acp{ied}, and Communication infrastructure~\cite{yadav2021architecture,klaer2020graphbased}.
Despite the stable nature of these systems allowing for signature monitoring to spot irregularities, their distinctive architecture calls for specialized protective measures against cyberattacks.
A weakness of existing research lies in its focus on network-level attacks, underestimating the impact of local communication devices and human operators, central to \ac{scada} operations.
%
%\mh{Hier wird mir die Struktur unklar. Background und Argumentation zu \ac{scada} kaufe ich, aber Process Memory und USB Drives fallen hier vom Himmel (und wurden auch im Glue Text nicht angeteasert). Evtl. B-D in eine Subsection zu HIDS mit entsprechenden Subsubsections zusammenfassen und am Anfang der Subsection etwas mehr Kontext geben?}
\subsection{HIDS Approach} \label{sec:hids}
\subsubsection{Process Memory} \label{subsec:process_memory}
The memory structures of a process are instrumental in identifying suspicious activities~\cite{angel2020disaggregation}.
When a process starts, the operating system forms a new address space divided into areas each serving distinct functions and possessing access attributes.
This division allows secure inter-process communication and synchronization~\cite{rrushi2022physics}.
A detailed inspection of these memory regions, especially the code segment, could reveal any altered or new malicious code, vital for systems' security.
Notably, most existing methods have focused on detecting malicious behavior based on network activity, often neglecting to analyze the memory of the processes running on the system.
Therefore, a method to scrutinize memory structures could contribute significantly to system security, especially in \ac{scada} environments.
%
\subsubsection{USB Drive} \label{subsec:usb_drive}
USB, a widespread peripheral communication standard, poses security challenges due to its lack of inherent security features~\cite{abou2021securing}.
As USB drives are prevalent in industrial control systems to personal computers, their insecure design could potentially aid malicious threats.
Typical USB-based threats exploit lacking authentication, where an untrusted device deceives the system into accepting it, leading to various malicious activities, including potential service disruption.
Unlike previous research, which primarily focuses on network-level attacks, considering threats emerging from insecure peripheral devices such as USB drives is also essential.
%
\subsubsection{Related Work} \label{subsec:related_work}
Several studies have centered on \ac{ids} for \ac{scada} systems, using different techniques to detect anomalies.
Anomaly detection relies on identifying deviations from typical system behavior, whereas pattern detection necessitates recognizing system behavior patterns that correspond to known attacks.
~\cite{suaboot2021holistic} presents a holistic data exfiltration detection approach, using supervised machine learning techniques, behavior-based detection, memory-based monitoring, and temporal data exfiltration detection for \ac{scada} systems.
A novel \ac{hids} framework proposed by~\cite{subba2021tfidfvectorizer} has shown effectiveness in real-time anomaly detection.
In~\cite{zhu2023industrial}, a model examining virus propagation within \ac{scada} systems is proposed, shedding light on potential control strategies.
The work of~\cite{gassais2020multi} proposes a host-based intrusion detection framework for smart devices in the \ac{iot}, combining machine learning algorithms and tracing techniques. 
Another work~\cite{moon2017dtb} presents an \ac{ids} using decision trees to detect and mitigate \ac{apt} attacks by analyzing network behavior and processes.
In the same direction, the work of~\cite{lee2023classification} analyzes \ac{apt} attack scenarios and techniques, classifies and analyzes malicious code detection methods, and provides insights for detecting and preventing malicious codes.
However, no previous research has targeted using USB device identification or process memory scanning and hashing as techniques for \ac{hids} in \ac{scada} systems. %\mh{Nur drei Paper related work wirkt etwas duenn}
%
\subsection{Problem Analysis} \label{subsec:problem_analysis} %\mh{Auch das wurde oben im Glue Text nicht angeteasert}
While various measures have been proposed for cyber defense in \ac{scada} systems, important challenges still persist, including the insecure design of commonly used peripheral communication standards such as USB, which can serve as a potential entry point for cyber threats, as demonstrated by incidents like the Stuxnet attack in Iran. 
Furthermore, neglecting to analyze process memory structures may lead to overlooking malicious alterations, which can have serious implications for system security. 
Most current methods focus primarily on network-level activity, often missing local threats posed by process memory hijacking via USB drives. 
To address these gaps and enhance the security of \ac{scada} systems, this paper aims to create a cohesive link between the insecurity of peripheral communication standards and the potential risk of process memory hijacking by incorporating USB device identification, process memory scanning, and hashing techniques into a comprehensive \ac{hids} for \ac{scada} systems.

%\mh{Die beiden Punkten wirkten arg beliebig und scheinen ja auch nicht viel miteinander zu tun zu haben. Besser herausarbeiten, warum man sich genau auf diese beiden stuerzen sollte}

